Sensitivity forecasts for the cosmological recombination radiation in the presence of foregrounds

The cosmological recombination radiation (CRR) is one of the inevitable $\Lambda$CDM spectral distortions of the cosmic microwave background (CMB). While it shows a rich spectral structure across dm-mm wavelengths, it is also one of the smallest signals to target. Here we carry out a detailed forecast for the expected sensitivity levels required to not only detect but also extract cosmological information from the CRR in the presence of foregrounds. We use ${\tt CosmoSpec}$ to compute the CRR including all important radiative transfer effects and modifications to the recombination dynamics. We confirm that detections of the overall CRR signal are possible with spectrometer concepts like ${\it SuperPIXIE}$. However, for real exploitation of the cosmological information, a $\simeq 50$ times more sensitive spectrometer is required. While extremely futuristic, this could provide independent constraints on the primordial helium abundance, $Y_p$, and probe the presence of extra relativistic degrees of freedom during BBN and recombination. Significantly improving the constraints on other cosmological parameters requires even higher sensitivity (another factor of $\simeq 5$) when considering a combination of a CMB spectrometer with existing CMB data. To a large part this is due to astrophysical foregrounds which interestingly do not degrade the constraints on $Y_p$ and $N_{\rm eff}$ as much. A future CMB spectrometer could thus open a novel way of probing non-standard BBN scenarios, dark radiation and sterile neutrinos. In addition, inflation physics could be indirectly probed using the CRR in combination with existing and forthcoming CMB anisotropy data.

==> outline_intro.tex <==
\begin{itemize}
    \item COBE first discovered deviations to the CMB blackbody -- CMB is great!
    \item Broad statements about distortions 
    \item Standard distortion: CMB non-thermal equilibrium has led to spectral distortions (i.e. mu and y)
    \item Many previous works on this, and even missions proposed? 
    \item One of the most important in cosmology (predicted by $\Lambda$CDM is CRR) -- cite Chluba2016 (which distortions does LCDM predict?)
    \item Previously recombination one of the most import ant (i.e. Peebles, Sunyaev) -- in these calculations, one of the crucial distortions --> Lyman alpha, 
    \item Dubrovnich -- also high end transitions, very important
    \item (all detials in the Schwarzschild lecture) 
    \item Initially calculations based on basic stuff (i.e. Dubrovnich and Stolyarev 1996, Rybicki \& dell’Antonio 1993, Kholupenko 2005 CRR paper)
    \item Then evolved into more accurately considered physical stuff (i.e. Chluba and JARM papers)
    \item Crucial steps in calc: resolving l states, non equilibrium (Chluba 2007 'Non eq. high substates')
    \item In addition, FB emission neglected (first included in Chluba 2006)
    \item Helium (specifcially neutral helium) non-hydrogenic spectrum, (fine structure and hyperfine)
    \item Dynamical hydrogen and helium (hydrogen absorption, Kholupenko 2007, Chluba  and JARM 2007/08, RM JC RS helium, Switzer 2007 just recombination dynamics (dynamics done by ES, recombination structure in JC adn RM paper, first discussion of double ionized helium -- on HeIII, electron scattering is very important, maybe talk about this )
    \item `While the computation of the spectrum is fully accounted for in 2010, the detailed calculation is too time consuming (sic). One of the steps to curtail this issue is the use of the spectral conductances (cite Yacine) and this is done fully in the CosmoSpec code'
    %New paragraph -- what can we learn
    \item 'One of the big questions is what we can learn from the cosmological recombination radiation.' Summarise T0 paper conclusions. Quote leading order dependencies  Can refer back to JCRM Helium paper on the dynamical behaviour of the lines. 'CRR dependent on the parameters' -- cite T0 paper -- 'affects the structure of hte lines' -- cite RM paper on helium -- 'non-standard physics can also affect the recombination radiation such as annihilation of DM and VFC' -- cite Chluba 2009/10 DM paper.
    % Be careful to cite the ones that mention other parameter dependenceiws, but JCRS 2007 did this first (T0)
    \item First questions: what is the detectability? (small signal, low number of baryons etc, ~nK correction to the broad CMB spectrum (check the previous reference)  -- two avenues: one from ground and another from space (cite Rao aPSera paper, Vincent Desjacques for space mission respectively)
    \item For high freq: space missions: foregrounds are the challenges. Most recnet calculations (Voyage2050 WP) SuperPIXIE could calculate 2sigma and Voyage2050 10sigma (emphasise! We did all that!) 
    %New paragraph
    \item Observability  of parameter dependencies: 1. Illustrated in T0 paper and CosmoSpec paper. 2. Calculations were slow: now we can do full estimates (back in 2007, interpolation was used for PICO cite Fendt RICO paper) -- already seeing some sensitivities. IN absence of foregrounds, Yp could be detected (cite Fendt thesis) (quote sensitivity)
    \item Neglecting FG: calculations refined (Khatri 2019, no more mention) 
    \item 
    
    \item In this paper...
\end{itemize}

==> tables-JC/spect_only_standard_neff_stat.tex <==
\begin{tabular}{llccc}
\toprule
Expt. & Analysis &  $\omb$ &  $\omc$ &  $\Neff$             \\
\midrule
\multirow{4}{*}{\Voyage} & No Frgs. &            42 &                     0.6 &               0.1 \\
            & Dist. Frgs. &            13 &                     0.5 &               0.1 \\
            & Astr. Frgs. &             7.3 &                     0.4 &            0.1 \\
            & $\textbf{All Frgs.}$ &             4.8 &                     0.4 &               0.1 \\
\cline{1-5}
\multirow{4}{*}{\Voyagep} & No Frgs. &           417 &                     5.6 &              1.2 \\
            & Dist. Frgs. &           135 &                     5.1 &       1.2 \\
            & Astr. Frgs. &            73 &                     4.3 &               1.1 \\
            & $\textbf{All Frgs.}$ &            48 &                     4.0 &            1.1 \\
\bottomrule
\end{tabular}


==> tables/spect_only_standard_neff_stat.tex <==
\begin{tabular}{llcccc}
\toprule
            &                      &  $\Omega_b h^2$ &  $\Omega_{\rm CDM} h^2$ &  $H_0$ &  $N_{\rm eff}$ \\
Expt. & Analysis &                 &                         &        &                \\
\midrule
\multirow{4}{*}{SUPER PIXIE} & No Frgs. &             8.1 &                     0.1 &    0.0 &            0.0 \\
            & Spec. Dist. Frgs. &             2.7 &                     0.1 &    0.0 &            0.0 \\
            & Astroph. Frgs. &             1.5 &                     0.1 &    0.0 &            0.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     0.1 &    0.0 &            0.0 \\
\cline{1-6}
\multirow{4}{*}{VOYAGE 2050} & No Frgs. &            40.5 &                     0.6 &    0.0 &            0.1 \\
            & Spec. Dist. Frgs. &            13.5 &                     0.5 &    0.0 &            0.1 \\
            & Astroph. Frgs. &             7.3 &                     0.4 &    0.0 &            0.1 \\
            & $\textbf{All Frgs.}$ &             4.8 &                     0.4 &    0.0 &            0.1 \\
\cline{1-6}
\multirow{4}{*}{VOYAGE 2050 X 10} & No Frgs. &           407.0 &                     5.6 &    0.0 &            1.2 \\
            & Spec. Dist. Frgs. &           134.8 &                     5.1 &    0.0 &            1.1 \\
            & Astroph. Frgs. &            73.3 &                     4.3 &    0.0 &            1.1 \\
            & $\textbf{All Frgs.}$ &            48.2 &                     4.0 &    0.0 &            1.1 \\
\bottomrule
\end{tabular}


==> tables/spect_only_standard_stat.tex <==
\begin{tabular}{llccc}
\toprule
            &                      &  $\Omega_b h^2$ &  $\Omega_{\rm CDM} h^2$ &  $H_0$ \\
Expt. & Analysis &                 &                         &        \\
\midrule
\multirow{4}{*}{SUPER PIXIE} & No Frgs. &             8.6 &                     0.4 &    0.0 \\
            & Spec. Dist. Frgs. &             2.7 &                     0.3 &    0.0 \\
            & Astroph. Frgs. &             1.5 &                     0.2 &    0.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     0.1 &    0.0 \\
\cline{1-5}
\multirow{4}{*}{VOYAGE 2050} & No Frgs. &            43.3 &                     2.1 &    0.0 \\
            & Spec. Dist. Frgs. &            13.7 &                     1.4 &    0.0 \\
            & Astroph. Frgs. &             7.4 &                     0.9 &    0.0 \\
            & $\textbf{All Frgs.}$ &             4.8 &                     0.7 &    0.0 \\
\cline{1-5}
\multirow{4}{*}{VOYAGE 2050 X 10} & No Frgs. &           430.3 &                    21.1 &    0.0 \\
            & Spec. Dist. Frgs. &           136.8 &                    13.6 &    0.0 \\
            & Astroph. Frgs. &            74.1 &                     8.9 &    0.0 \\
            & $\textbf{All Frgs.}$ &            48.2 &                     6.7 &    0.0 \\
\bottomrule
\end{tabular}


==> tables/spect_only_standard_yp_neff_stat.tex <==
\begin{tabular}{llccccc}
\toprule
            &                      &  $\Omega_b h^2$ &  $\Omega_{\rm CDM} h^2$ &  $H_0$ &  $Y_P$ &  $N_{\rm eff}$ \\
Expt. & Analysis &                 &                         &        &        &                \\
\midrule
\multirow{4}{*}{SUPER PIXIE} & No Frgs. &             7.2 &                     0.1 &    0.0 &    1.0 &            0.0 \\
            & Spec. Dist. Frgs. &             2.3 &                     0.1 &    0.0 &    0.8 &            0.0 \\
            & Astroph. Frgs. &             1.3 &                     0.1 &    0.0 &    0.5 &            0.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     0.1 &    0.0 &    0.4 &            0.0 \\
\cline{1-7}
\multirow{4}{*}{VOYAGE 2050} & No Frgs. &            35.8 &                     0.5 &    0.0 &    4.8 &            0.1 \\
            & Spec. Dist. Frgs. &            11.5 &                     0.5 &    0.0 &    3.9 &            0.1 \\
            & Astroph. Frgs. &             6.3 &                     0.4 &    0.0 &    2.5 &            0.1 \\
            & $\textbf{All Frgs.}$ &             4.8 &                     0.3 &    0.0 &    2.0 &            0.1 \\
\cline{1-7}
\multirow{4}{*}{VOYAGE 2050 X 10} & No Frgs. &           359.5 &                     5.5 &    0.0 &   47.7 &            1.2 \\
            & Spec. Dist. Frgs. &           115.6 &                     5.0 &    0.0 &   38.8 &            1.1 \\
            & Astroph. Frgs. &            62.8 &                     3.9 &    0.0 &   25.3 &            1.0 \\
            & $\textbf{All Frgs.}$ &            48.1 &                     3.3 &    0.0 &   20.5 &            1.0 \\
\bottomrule
\end{tabular}


==> tables/spect_only_standard_yp_stat.tex <==
\begin{tabular}{llcccc}
\toprule
            &                      &  $\Omega_b h^2$ &  $\Omega_{\rm CDM} h^2$ &  $H_0$ &  $Y_P$ \\
Expt. & Analysis &                 &                         &        &        \\
\midrule
\multirow{4}{*}{SUPER PIXIE} & No Frgs. &             7.4 &                     0.4 &    0.0 &    1.0 \\
            & Spec. Dist. Frgs. &             2.3 &                     0.3 &    0.0 &    0.8 \\
            & Astroph. Frgs. &             1.3 &                     0.2 &    0.0 &    0.6 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     0.1 &    0.0 &    0.4 \\
\cline{1-6}
\multirow{4}{*}{VOYAGE 2050} & No Frgs. &            37.3 &                     1.8 &    0.0 &    4.8 \\
            & Spec. Dist. Frgs. &            11.6 &                     1.3 &    0.0 &    3.9 \\
            & Astroph. Frgs. &             6.3 &                     0.9 &    0.0 &    2.7 \\
            & $\textbf{All Frgs.}$ &             4.8 &                     0.6 &    0.0 &    2.2 \\
\cline{1-6}
\multirow{4}{*}{VOYAGE 2050 X 10} & No Frgs. &           373.7 &                    18.2 &    0.0 &   47.8 \\
            & Spec. Dist. Frgs. &           115.9 &                    13.4 &    0.0 &   39.2 \\
            & Astroph. Frgs. &            62.9 &                     8.6 &    0.0 &   27.1 \\
            & $\textbf{All Frgs.}$ &            48.2 &                     5.8 &    0.0 &   21.8 \\
\bottomrule
\end{tabular}


==> tables/spect_planck_standard_neff_stat.tex <==
\begin{tabular}{llcccc}
\toprule
            &                      &  $\Omega_b h^2$ &  $\Omega_{\rm CDM} h^2$ &  $H_0$ &  $N_{\rm eff}$ \\
Expt. & Analysis &                 &                         &        &                \\
\midrule
\multirow{4}{*}{SUPER PIXIE} & No Frgs. &             1.0 &                     1.0 &    1.0 &            1.0 \\
            & Spec. Dist. Frgs. &             1.0 &                     1.0 &    1.0 &            1.0 \\
            & Astroph. Frgs. &             1.0 &                     1.0 &    1.0 &            1.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     1.0 &    1.0 &            1.0 \\
\cline{1-6}
\multirow{4}{*}{VOYAGE 2050} & No Frgs. &             0.9 &                     1.0 &    0.9 &            1.0 \\
            & Spec. Dist. Frgs. &             1.0 &                     1.0 &    1.0 &            1.0 \\
            & Astroph. Frgs. &             1.0 &                     1.0 &    1.0 &            1.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     1.0 &    1.0 &            1.0 \\
\cline{1-6}
\multirow{4}{*}{VOYAGE 2050 X 10} & No Frgs. &             0.2 &                     0.7 &    0.5 &            0.6 \\
            & Spec. Dist. Frgs. &             0.5 &                     0.9 &    0.7 &            0.8 \\
            & Astroph. Frgs. &             0.7 &                     0.9 &    0.8 &            0.9 \\
            & $\textbf{All Frgs.}$ &             0.8 &                     1.0 &    0.9 &            0.9 \\
\bottomrule
\end{tabular}


==> tables/spect_planck_standard_stat.tex <==
\begin{tabular}{llccc}
\toprule
            &                      &  $\Omega_b h^2$ &  $\Omega_{\rm CDM} h^2$ &  $H_0$ \\
Expt. & Analysis &                 &                         &        \\
\midrule
\multirow{4}{*}{SUPER PIXIE} & No Frgs. &             1.0 &                     1.0 &    1.0 \\
            & Spec. Dist. Frgs. &             1.0 &                     1.0 &    1.0 \\
            & Astroph. Frgs. &             1.0 &                     1.0 &    1.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     1.0 &    1.0 \\
\cline{1-5}
\multirow{4}{*}{VOYAGE 2050} & No Frgs. &             0.9 &                     1.0 &    1.0 \\
            & Spec. Dist. Frgs. &             1.0 &                     1.0 &    1.0 \\
            & Astroph. Frgs. &             1.0 &                     1.0 &    1.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     1.0 &    1.0 \\
\cline{1-5}
\multirow{4}{*}{VOYAGE 2050 X 10} & No Frgs. &             0.3 &                     0.8 &    0.7 \\
            & Spec. Dist. Frgs. &             0.5 &                     0.8 &    0.7 \\
            & Astroph. Frgs. &             0.6 &                     0.8 &    0.8 \\
            & $\textbf{All Frgs.}$ &             0.8 &                     0.9 &    0.8 \\
\bottomrule
\end{tabular}


==> tables/spect_planck_standard_yp_neff_stat.tex <==
\begin{tabular}{llccccc}
\toprule
            &                      &  $\Omega_b h^2$ &  $\Omega_{\rm CDM} h^2$ &  $H_0$ &  $Y_P$ &  $N_{\rm eff}$ \\
Expt. & Analysis &                 &                         &        &        &                \\
\midrule
\multirow{4}{*}{SUPER PIXIE} & No Frgs. &             1.0 &                     1.0 &    1.0 &    1.0 &            1.0 \\
            & Spec. Dist. Frgs. &             1.0 &                     1.0 &    1.0 &    1.0 &            1.0 \\
            & Astroph. Frgs. &             1.0 &                     1.0 &    1.0 &    1.0 &            1.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     1.0 &    1.0 &    1.0 &            1.0 \\
\cline{1-7}
\multirow{4}{*}{VOYAGE 2050} & No Frgs. &             0.9 &                     0.9 &    0.9 &    0.9 &            0.9 \\
            & Spec. Dist. Frgs. &             1.0 &                     1.0 &    1.0 &    0.9 &            1.0 \\
            & Astroph. Frgs. &             1.0 &                     1.0 &    1.0 &    0.9 &            1.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     1.0 &    1.0 &    1.0 &            1.0 \\
\cline{1-7}
\multirow{4}{*}{VOYAGE 2050 X 10} & No Frgs. &             0.3 &                     0.6 &    0.5 &    0.3 &            0.5 \\
            & Spec. Dist. Frgs. &             0.6 &                     0.6 &    0.6 &    0.3 &            0.6 \\
            & Astroph. Frgs. &             0.8 &                     0.7 &    0.7 &    0.3 &            0.7 \\
            & $\textbf{All Frgs.}$ &             0.9 &                     0.8 &    0.8 &    0.4 &            0.8 \\
\bottomrule
\end{tabular}


==> tables/spect_planck_standard_yp_stat.tex <==
\begin{tabular}{llcccc}
\toprule
            &                      &  $\Omega_b h^2$ &  $\Omega_{\rm CDM} h^2$ &  $H_0$ &  $Y_P$ \\
Expt. & Analysis &                 &                         &        &        \\
\midrule
\multirow{4}{*}{SUPER PIXIE} & No Frgs. &             1.0 &                     1.0 &    1.0 &    1.0 \\
            & Spec. Dist. Frgs. &             1.0 &                     1.0 &    1.0 &    1.0 \\
            & Astroph. Frgs. &             1.0 &                     1.0 &    1.0 &    1.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     1.0 &    1.0 &    1.0 \\
\cline{1-6}
\multirow{4}{*}{VOYAGE 2050} & No Frgs. &             0.9 &                     1.0 &    1.0 &    1.0 \\
            & Spec. Dist. Frgs. &             1.0 &                     1.0 &    1.0 &    1.0 \\
            & Astroph. Frgs. &             1.0 &                     1.0 &    1.0 &    1.0 \\
            & $\textbf{All Frgs.}$ &             1.0 &                     1.0 &    1.0 &    1.0 \\
\cline{1-6}
\multirow{4}{*}{VOYAGE 2050 X 10} & No Frgs. &             0.3 &                     0.8 &    0.6 &    0.3 \\
            & Spec. Dist. Frgs. &             0.6 &                     0.9 &    0.7 &    0.4 \\
            & Astroph. Frgs. &             0.8 &                     0.9 &    0.9 &    0.5 \\
            & $\textbf{All Frgs.}$ &             0.8 &                     0.9 &    0.9 &    0.6 \\
\bottomrule
\end{tabular}

